The Multi-fidelity Multi-armed Bandit

We study a variant of the classical stochastic $K$-armed bandit where observing the outcome of each arm is expensive, but cheap approximations to this outcome are available. For example, in online advertising the performance of an ad can be approximated by displaying it for shorter time periods or to narrower audiences. We formalise this task as a multi-fidelity bandit, where, at each time step, the forecaster may choose to play an arm at any one of $M$ fidelities. The highest fidelity (desired outcome) expends cost $\lambda^{(m)}$. The $m^{\text{th}}$ fidelity (an approximation) expends $\lambda^{(m)} < \lambda^{(M)}$ and returns a biased estimate of the highest fidelity. We develop MF-UCB, a novel upper confidence bound procedure for this setting and prove that it naturally adapts to the sequence of available approximations and costs thus attaining better regret than naive strategies which ignore the approximations. For instance, in the above online advertising example, MF-UCB would use the lower fidelities to quickly eliminate suboptimal ads and reserve the larger expensive experiments on a small set of promising candidates. We complement this result with a lower bound and show that MF-UCB is nearly optimal under certain conditions.

==> _ <==


\section{Some Simulations on Synthetic Problems}
\label{sec:simulations}

We compare \ucbs against \mfucbs on a series of synthetic problems.
The results are given in Figure~\ref{fig:sim}.
Due to space constraints, the details on these experiments are given in
Appendix~\ref{app:simulations}.

We have also illustrated the number of plays by \mfucbs and \ucbs at each fidelity
 for one of these problems. 
Note that while \mfucbs has several plays at suboptimal arms they don't cost as much.

\insertSimOneFigure

% In Figures~\ref{fig:K100}-\ref{fig:K200B} we construct problems with various values
% for $M,K$ and the costs $\{\costm\}_{m=1}^M$. Figures~\ref{fig:K100},~\ref{fig:K500}
% use Gaussian rewards while Figure~\ref{fig:K200B} uses Bernoulli rewards.
% While there seems to be an optimal value for $\gamma$ for a given problem, 
% \mfucbs beats \ucbs for a large range of values of $\gamma$.
% 
% An \emph{interesting observation} in most figures is that for small $\gamma$, 
% there is an initial
% phase of linear regret after which the regret improves significantly.
% In these cases, \mfucbs uses several plays at the lower fidelities (due to the small
% choice of $\gamma$) during which it receives $0$ reward.
% However, as $\gamma$ is small, it is able to focus on a very small set once it starts
% playing at the highest fidelity.
% Therefore, the regret improves, often outperforming larger $\gamma$ values. 
% This behaviour aligns well with our theoretical findings.
% We also see that when $\gamma$ is very large, \mfucbs approaches the performance of \ucb.
% 
% In the simulations shown we used $\rho=3.01$ for \mfucbs and $\rho=2.01$ for \ucbs (see
% Theorem 2.1 of~\citet{bubeck12regret}). However, all methods performed better for
% more aggressive choices of $\rho$.
% The experiments in Figures~\ref{fig:K100}-\ref{fig:K200B} were constructed so that
% $|\Kcalupm|$ was approximately $20\%$ of $|\Kcalm\cup\Kcalupm|$.
% For example in Fig.~\ref{fig:K500}, $\approx 100$ arms had
% $\Deltaonek=\muMopt-\muonek-\zetaone<0$ of which
% $\approx 20$ arms had $\Deltatwok<0$ and $\approx 4$ had $\Deltammkk{3}{k}<0$.
% All curves were produced by averaging over $10$ experiments. The error bars are not
% visible since they are too small.



==> appMainThms.tex <==

\section{Proofs of Theorems~\ref{thm:RcBound} \&~\ref{thm:RsBound}}
\label{app:mainThms}

We now instantiate Lemma~\ref{lem:ERCOSTBound} to obtain bounds for $\Rc$ and $\Rs$.

\begin{proof}[\textbf{Proof of Theorem~\ref{thm:RcBound}}]
Recall that $\psigammam = \frac{\costm}{\costmm{m+1}}\psi(\zetam)$ and 
$\omegamk = \DeltaMk$. Plugging this into Lemma~\ref{lem:ERCOSTBound} 
we get
\begin{align*}
\EE[\Rc(\COST)] &\leq\; \muMopt \costM \;+\;
  \sum_{k=1}^K \DeltaMk\left(
    \sum_{\ell=1}^{[k]-1}\costmm{\ell+1} \frac{\rho\lognlpc}{\psizetal}
  \;\;+\; \costkmap \frac{\rho\lognlpc}{\psiDeltakmapk} 
  \;+\kapparho\costM
  \right) \\
  &\leq\; 
\muMopt \costM \;+\;
  \sum_{k=1}^K \DeltaMk\cdot\costkmap\rho\lognlpc 
  \left( \frac{2}{\psizetakmapmo}
  + \frac{1}{\psiDeltakmapk} \right)
  + \DeltaMk\kapparho\costM
\end{align*}
The second step uses Assumption~\ref{asm:decayCondn}.
The theorem follows by noting that for any $k\in\Kcalm$ and $\ell<m$,
$\Deltamk  = \Deltalk + \zetal - \zetam + \mulk-\muMk + \muMk-\mumk
\leq 2\gammal + 2\zetal \leq 4\zetal$.
Therefore $1/\psiDeltamkb > c_1/\psi(\zetal)$ where $c_1$ depends on $\psi$ (for
sub-Gaussian distributions, $c_1=1/16$).
\end{proof}


\begin{proof}[\textbf{Proof of Theorem~\ref{thm:RsBound}}]
The proof follows similar to above.
Recall that $\psigammam = \frac{\costm}{\costmm{m+1}}\frac{\psi(\zetam)}{\zetam/B}$ 
and  $\omegaMk = \DeltaMk$, $\omegamk = \muMopt$ for $m<M$. 
Plugging this into Lemma~\ref{lem:ERCOSTBound} and using 
Assumption~\ref{asm:decayCondn} and $\muMopt \leq B$
we have
\begin{align*}
\EE[\Rs(\COST)] &\leq\; \muMopt \costM \;+\;
  \sum_{k\in \optArms}  
  \costM\rho\lognlpc  \frac{\zetamm{M-1}}{\psi(\zetamm{M-1}}
  \\ 
  &\hspace{0.2in}
  \sum_{k\in \cup\Kcalm} \costM\rho\lognlpc
  \left(\frac{\zetamm{M-1}}{\psi(\zetamm{M-1}}
  \;+\;
     \frac{\DeltaMk}{\psi(\DeltaMk/2)}
  \right)
  \\ 
  &\hspace{0.2in}
  \sum_{k\notin \Kcalm\cup\optArms}  \costkmap\rho\lognlpc\left(
  \frac{2\zetakmapmo}{\psizetakmapmo}
  \;+\; \frac{\muMopt}{\psiDeltakmapk}
  \;+\; \muMopt\kapparho\costM
  \right)
\end{align*}
% The second step uses Assumption~\ref{asm:decayCondn}.
As before the theorem follows by noting that $\Deltamk < 4\zetal$ for $k\in\Kcalm$
and $\ell<m$ using Assumption~\ref{asm:decayCondn}.
Therefore for $\ell<m<M$,  
$\frac{\muMopt}{\psiDeltamkb} \gtrsim 
\frac{\muMopt}{\psizetal} \gtrsim \frac{\zetal}{\psizetal} $.
For $m=M$, using that $x/\psi(x)$ is decreasing in $x$ we have,
$\frac{\DeltaMk}{\psiDeltaMkb} \gtrsim 
\frac{\zetal}{\psizetal}$.
\end{proof}



